Finding Transformer Circuits with Edge Pruning

The path to interpreting a language model often proceeds via analysis of circuits -- sparse computational subgraphs of the model that capture specific aspects of its behavior. Recent work has automated the task of discovering circuits. Yet, these methods have practical limitations, as they rely either on inefficient search algorithms or inaccurate approximations. In this paper, we frame automated circuit discovery as an optimization problem and propose *Edge Pruning* as an effective and scalable solution. Edge Pruning leverages gradient-based pruning techniques, but instead of removing neurons or components, it prunes the \emph{edges} between components. Our method finds circuits in GPT-2 that use less than half the number of edges compared to circuits found by previous methods while being equally faithful to the full model predictions on standard circuit-finding tasks. Edge Pruning is efficient even with as many as 100K examples, outperforming previous methods in speed and producing substantially better circuits. It also perfectly recovers the ground-truth circuits in two models compiled with Tracr. Thanks to its efficiency, we scale Edge Pruning to CodeLlama-13B, a model over 100x the scale that prior methods operate on. We use this setting for a case study comparing the mechanisms behind instruction prompting and in-context learning. We find two circuits with more than 99.96% sparsity that match the performance of the full model and reveal that the mechanisms in the two settings overlap substantially. Our case study shows that Edge Pruning is a practical and scalable tool for interpretability and sheds light on behaviors that only emerge in large models.

==> appendices/pruning.tex <==
\label{ap:pruning}
Our formulation of pruning is based on that used by CoFi Pruning~\citep{xia-etal-2022-structured}.
Specifically, we model the masks $\boldsymbol{z}$ based on the hard concrete distribution as done by~\citet{louizos2018learning}:
$$\mathbf{u} \sim \text{Uniform}(\epsilon,1-\epsilon)$$
$$\textbf{s} = \sigma\left(\frac{1}{\beta} \cdot \frac{\mathbf{u}}{1-\mathbf{u}} + \log \boldsymbol{\alpha}\right)$$
$$\tilde{\mathbf{s}} = \mathbf{s} \times (r-l) + l$$
$$\mathbf{z} = \min(1, \max(0, \tilde{\mathbf{s}}))$$
where $\sigma$ refers to the sigmoid function,  $\epsilon = 10^{-6}$, and
$\log \boldsymbol{\alpha}$ indicates that the logarithm is applied element-wise.
We fix the temperature $\frac{1}{\beta} = \frac{2}{3}$.
The last two lines stretch the distribution to $[l, r] = [-0.1, 1.1]$ and accumulate the ``excess'' probability on either side to $0$ and $1$, respectively.
The log alphas $\log \boldsymbol{\alpha}$ are the learnable parameters in this formulation.

Following, \citet{wang-etal-2020-structured}, a target sparsity is enforced via a Lagrangian term~\citep{louizos2018learning}. 
If the current sparsity is $s$, the term, parametrized by a reference value $t$ is
$$\mathcal L_s = \lambda_1 \cdot (t-s) + \lambda_2 \cdot (t-s)^2$$
$\lambda_1$ and $\lambda_2$ are also updated during training via gradient \emph{ascent} to keep the regularization tight.
We vary the value of $t$ throughout training, linearly increasing it from $0$ to a target value, as outlined in Appendix~\ref{ap:hparams}.
Although it may be useful to think of $t$ as a ``target'' sparsity, it is only a number.
The runs usually converge to a value slightly below $t$, so it is prudent to set it to a value \emph{greater than} $1$---although $s$ can then never reach the target value, it will be pushed to higher sparsities.

We have two sets of masks $z$.
The first set associates a $0-1$ value $z_e$ with each edge $e \equiv (n_1, n_2)$ in the computational graph.
The second set tags each \emph{node} of the graph $n$ with a $0-1$ value $z_n$.
The latter specifies whether a node is ``active'', i.e., producing output.
In effect, the presence of an edge $e \equiv (n_1, n_2)$ is determined by the binary mask
$$\tilde{z}_{(n_1, n_2)} = z_{(n_1, n_2)} \times z_{n_1}$$
We initially only used edge masks but found that the method would have difficulty converging to high sparsities (i.e., end up at low sparsities).
Introducing a second set of masks allows the process to eliminate many edges quickly, accelerating the removal of unimportant components.
However, the lagrangian above only applies to the edge masks. 
This is fine since the node masks can only remove further edges, not introduce new ones on top of those chosen by the edge masks.
The final loss is
$$\mathcal L = \mathcal L_{\text{KL}} + \mathcal L_{\text{edge}, s}$$

